Balancing Reinforcement Learning Training Experiences in Interactive Information Retrieval

Interactive Information Retrieval (IIR) and Reinforcement Learning (RL) share many commonalities, including an agent who learns while interacts, a long-term and complex goal, and an algorithm that explores and adapts. To successfully apply RL methods to IIR, one challenge is to obtain sufficient relevance labels to train the RL agents, which are infamously known as sample inefficient. However, in a text corpus annotated for a given query, it is not the relevant documents but the irrelevant documents that predominate. This would cause very unbalanced training experiences for the agent and prevent it from learning any policy that is effective. Our paper addresses this issue by using domain randomization to synthesize more relevant documents for the training. Our experimental results on the Text REtrieval Conference (TREC) Dynamic Domain (DD) 2017 Track show that the proposed method is able to boost an RL agent's learning effectiveness by 22\% in dealing with unseen situations.

==> intro.tex <==

\section{Introduction}

%Deep reinforcement learning (DRL) is one of the most promising domains in machine learning. %It has achieved great success in a broad range of fields, including video games \citep{DQN}, board games \citep{AlphaGo2} and robotics \citep{RL_robotics_surbey}. 
%A general DRL algorithm first runs its policy to generate a set of trajectories. The generated trajectories are used to estimate returns or to fit a transition model, so as to improve the policy. The training repeats until the algorithm finds a good policy.  
%The generated trajectories are the basis for the success of a DRL algorithm. Those trajectories usually can be easily obtained when the environment is characterized by explicitly-defined rules or physical laws, such as games and robotic simulators. However, sometimes, obtaining those trajectories could become quite expensive when the agent-environment interaction requires human participation \citep{human_rl}. Examples include recommendation system,  conversational search systems and self-driving cars. %This challenge is becoming more and more severe as the neural net is growing deeper and deeper every day. Due to the expensive interaction process, only minimal trajectory data is available for training. 

Simulated training helps reinforcement learning (RL) when it is costly or unrealistic to obtain real-world training data. It creates simulations to augment original learning environments and help reduce sample complexity for the training. When deploying an simulation-trained RL agent to a real-world unseen environment, the challenge is how to transfer from simulations to reality and close the `reality gap', i.e. the discrepancy between the reality and the simulator \citep{collins2019quantifying}. One idea is to increase the generalization ability of the agent by {\it domain randomization}. Assuming randomized environments would cover more samples from the true distribution, domain randomization works by randomizing variables in available training environments and derives more diversified environments. It has been studied in domains such as  robotics \citep{sadeghi2016cad2rl} and vision \citep{tremblay2018training}, however, few attempts have been made in textual domains. 

%One of them is referred as reality gap, i.e. the discrepancy between the reality and simulator \cite{}. Such differences prevent researchers from deploying an RL agent trained in simulated environments to the real environment without any adaptation.

% Because those limited trajectories lack diversity, it makes the training algorithm suffer from the issue of high variance. An agent may easily get stuck in a local optimum and is unable to find a good global policy. This costly agent-environment interaction prevents the RL agent to reach its full potential. 

 %Most of these textual domains are used in web-scale applications. Because the web is so dynamic, these applications require the trained RL agent to be able to generalize to unseen environments. However, at the scale of the Web, it is so costly and thus nearly impossible to obtain human feedback in real-time to train the RL agent. 
 
 In the text domain, an important task is to triage  information via multi-turn interactions with users. This includes applications such as online recommendation, dialogue systems, multi-turn question answering and dynamic search \citep{Yang:2016}. Most of them are web applications and face two major challenges. First, the web is so dynamic and constantly changing that an RL agent would most likely face unseen environment in test time. Second, the web has an enormous scale and it makes obtaining live feedback (reward) from real users very expensive, especially in small or non-commercial research institutions. 
 
%An example task is dynamic search \citep{Yang:2016}. Through continuous interactions with real-users, an RL agent finds out relevant documents from irrelevant documents. The user provides either implicit or explicit feedback that reflects the user's preferences regarding documents that the RL agent has already found. Relevant documents and irrelevant documents  can be seen as two classes of documents. The triage task is to separate them by interacting with the user (environment) to get many runs of feedback (reward). 

These information triage tasks can be characterized as the following. First, there are two classes of items in its data set -- dynamic search has relevant documents vs. irrelevant documents, question answering has correct vs. incorrect answers, and recommendation has things to recommend and things not. Second, the goal is to separate one class from the other. Third, however, the criteria (boundary) to distinguish the two classes are not very clear, at least at the beginning of the process. Fourth, the agent needs to find out the boundary via getting feedback from the environment through interactions. Fifth, eventually, the agent should be able to separate the items into different classes. 

For tasks under environment with such a two-class modality, a desirable RL method should be able to 1) help distinguish the boundary between the two classes, and 2) promote the more rare class (usually the positive class) to be found easier. 


%The training of the RL agent is usually done offline, with limited amount of annotated data. After training, the RL agent can then be deployed to the real environment. However, the repository may be updated every second. The trained RL agent may encounter documents that it has never seen before, which prevents it from achieving good performance in the deployment environment.
%As the environment emerges and changes every day, acquiring and annotating new training data would be unrealistic. Such situation requires us to train an RL agent that is able to   generalize from a limited amount of training trajectories.


In this paper, we propose a novel domain randomization method, {\it Document Environment Generation (DEG)},  to enhance reinforcement learning in text domains.  In our method, we propose to automatically create new learning environments to provide simulated training. The training process includes a stream of artificial environments that are similar to but different from the available real ones, which encourages the agent to generalize its learned policies.  We experiment with our method on the Text REtrieval Conference (TREC) Dynamic Domain Track (DD) and the results show that the proposed algorithm is able to boost the agents' learning effectiveness by 28\% in unseen environments.



==> new.tex <==
\section{New Training Method}

let $e_i$ = the ith generated synthetic environment 
The training method in current paper is :
original environment(1st)-$e_1$-$e_2$-$e_3$-.....$e_n$

New way:
select the next environment to train based on score S.

S = r(average improvement rate) + x(exploration rate)      

This formula of score S is like UCT in MCTS (Monte Carlo tree search).
after training on $e_i$, evaluate how it helps improve the performance of agent on the test environment, the improvement rate is r.
If r>10\%, that synthetic environment is store in a buffer to be signed as $e_i$. 
Thus, in the buffer, there are a lot of historically synthetic environments with average improvement rate > 10\%, and the original environment and the unseen new environment. Each environment owns a score S. We apply the softmax function to the S score of each environment to assign each environment a probability to be selected as the next training environment. If the unseen new environment is selected, a new environment will be generated to train the agent. Once the r(average improvement rate) of a specific environment is lower than 10\%, that environment will be removed from the buffer. However, the original environment and the unseen new environment will never be removed from the buffer. So it will be a infinite open-ended training process.



==> old.tex <==
\begin{comment}
\subsection{Why need more environments?}
In most of the DRL project, the environment we design is not as comprehensive as what it should be in the tasks. It cannot reflect all the information of the task. So we need a more informative, comprehensive and realistic representation to be our desire environment. That thing is a group of environments, which can diversely represent as much information as the task have.


The environment in most of the DRL tasks are not fixed, but emerges and changes with certain probability value. For example in self-driving cars, if we make the picture took by the central front camera as the environment of the DRL framework, the cars,  weather and items in the picture would definitely changes with different probability value, instead of only a fixed pattern. So no only do we need more and more pictures for our DRL agent to converge, but we also need more and more diverse pictures to embody the whole information of  what front camera will see. A high diversity of environments can also prevent the agent get sunk into a specific situation, prevent a ``overfit'' problem. 

So We treat the environment $e$ as a random variable. The distribution of a specific task is set to be $T$. $e\sim T$

However, in some case the environment is not easy to sample because of money, time and so on. With only a limit number of environments, or sometimes even only one environment with no change and diversity, like the continuous control tasks in MuJoCo,
we cannot train a walking agent in such a fixed environment with no diversity and transfer this agent into the road of real world. So what we can do is to enhance the diversity of its environment by increasingly generating diverse environments. An agent is easier to adapt to realistic environment if trained on a more diverse range of environments. Thus, in Dynamic Search tasks, where it is very expensive to sample a human-involved environment, the DEG algorithm can help enhance the textual diversity of environments.
\end{comment}

==> rl4ds.tex <==

\section{Reinforcement Learning Framework in Dynamic Search}
Dynamic search (DS) \citep{Yang:2016} models the scenario where a human user searches for relevant information in an iterative and interactive manner. Researchers have been making progress in this task by employing RL algorithms to optimize search engine's behavior. In this paper, we generally follow the framework in CE3 \citep{zhiwen}, one of the state-of-the-art DS systems based on Proximal Policy Optimization (PPO) \citep{PPO}. We adopt its variant which uses Doc2Vec \citep{doc2vec} representation because of efficiency.  


% \subsection{Dynamic Search Background}
% 这里要把 corpus， doc等DS概念抛出，才能在之后的 得抬

In DS, the search system attempts to satisfy user's information need by trial-and-error. The human user provides the initial description of the information need. Then at each timestep, the search system retrieves a set of documents from the text corpus and return it to the user. The user provides explicit or implicit feedback regarding the documents received. The search system then adjust its search algorithm and repeat the above process. Such interaction continues until the user's information need is satisfied.

The human user, along with the text corpus, constitute the environment which the RL agent, i.e. the search system, interacts with. We formulate the state, action and reward for the RL agent following \citep{zhiwen}. 

\begin{figure*}
    \centering
    \includegraphics[width=1.1\textwidth]{fig/Generate_doc.png}
    \caption{Generate a specific new document}
    \label{fig:my_label1}
\end{figure*}


\subsection{Action}
% The insight of the action calculation function is derived from [zhiwen’s paper].
% 询问zhiwen action 细节才能捋清写公式，目前猜想 costomer network 直接出 action ？ 另外：diversity的如果2w部的快速结果不好需要重做5w部的实验，以及diversity的图像显示并不是每次都mean上涨

The action of the RL agent is a vector of $n$ dimension, which is the output of policy network. The relevance score of each document is computed by summing over the dot products between the action vector and every segment vector in this document. After that, top-scored documents are returned to the user.



\subsection{Reward}
The reward of the agent's action is the sum of relevance ratings of returned documents. Those relevance ratings are from third-party assessors, where 4 means key results, 3 means highly relevant and 0 means non-relevant. 
